Hierarchical Cut Labelling -- Scaling Up Distance Queries on Road Networks

Answering the shortest-path distance between two arbitrary locations is a fundamental problem in road networks. Labelling-based solutions are the current state-of-the-arts to render fast response time, which can generally be categorised into hub-based labellings, highway-based labellings, and tree decomposition labellings. Hub-based and highway-based labellings exploit hierarchical structures of road networks with the aim to reduce labelling size for improving query efficiency. However, these solutions still result in large search spaces on distance labels at query time, particularly when road networks are large. Tree decomposition labellings leverage a hierarchy of vertices to reduce search spaces over distance labels at query time, but such a hierarchy is generated using tree decomposition techniques, which may yield very large labelling sizes and slow querying. In this paper, we propose a novel solution \emph{hierarchical cut 2-hop labelling (HC2L)} to address the drawbacks of the existing works. Our solution combines the benefits of hierarchical structures from both perspectives - reduce the size of a distance labelling at preprocessing time and further reduce the search space on a distance labelling at query time. At its core, we propose a new hierarchy, \emph{balanced tree hierarchy}, which enables a fast, efficient data structure to reduce the size of distance labelling and to select a very small subset of labels to compute the shortest-path distance at query time. To speed up the construction process of HC2L, we further propose a parallel variant of our method, namely HC2L$^p$. We have evaluated our solution on 10 large real-world road networks through extensive experiments.

==> section_Algorithms.tex <==
\begin{comment}


\begin{figure}[h]
\centering
\includegraphics[scale=0.6]{img/nb.pdf}

\caption{Binary tree hierarchy.}
\label{fig:Btree_hierarchy}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[scale=0.55]{img/nb_decomposition.pdf}

\caption{Binary tree structure of the network in Figure 1.}
\label{fig:Btree_structure}
\end{figure}


% \begin{figure*}[h]
% \centering

% \includegraphics[scale=0.49]{img/td.pdf}
% \hspace*{0.2cm}
% \includegraphics[scale=0.49]{img/nb_lca.pdf}

% \caption{Tree decomposition of the network in Figure 1.}
% \label{fig:td_structure}
% \end{figure*}









\section{Binary Tree Construction}
%In this section, we introduce an algorithm which, given a graph $G$, produces a near-balanced tree decomposition $T_G$ efficiently. This enables us to compute a near-balanced tree hierarchy of vertices in a road network.

Given a road network, there may exist many binary tree hierarchies which satisfy Definition~\ref{def:td}. However, we are mainly interested in a binary tree hierarchy in which the set of vertices in each node is as small as possible and represent a vertex cut on the corresponding distance-preserving subgraph. Finding a small vertex cut set that partitions the graph into two components of similar size lies at the core of our approach which is closely related to \emph{the minimum balanced vertex separator problem}, and is known to be NP-hard.
% This leads to close connections to \emph{the minimum balanced vertex separator problem}, which is known to be NP-hard~\cite{?}. %Finding a small vertex cut set that partitions the graph into two components of similar size lies at the core of our approach.
%This is known as \emph{the minimum balanced vertex separator problem}, which is NP-hard. 
Various heuristic and approximation algorithms for the minimum balanced vertex separator problem exist -- in particular, balanced cuts containing at most $O(\sqrt{V})$ vertices can be efficiently found for planar graphs \cite{doi:10.1137/0136016}. However, we are interested in partitions that are not only balanced, but also self-contained with respect to shortest paths. That is, the distance between two nodes within a partition should be the same as the distance in the full graph, for as many nodes as possible, to minimize the number of shortcut insertions needed. Hence, we devise our own heuristic approach, which we describe in the following.

%\q{(Discuss two additional requirements from the 2-hop labelling perspective and the corresponding algorithmic challenges on top of near-balanced tree decomposition: minimizing vertex cuts and preserving distance)}

\subsection{Small Balanced Cuts}
In this section, we shall introduce our proposed partitioning algorithm which can efficiently decompose a road network into a binary tree structure.

The basic idea is to start with a rough partition of the graph into three components: two initial partitions $P'_A, P'_B$, which are connected via a third partition that we shall refer to as a \emph{middle partition}.
We then find a minimal vertex cut within the middle partition, as illustrated in Figure~\ref{fig:vertex-cut}. Containment of the initial partitions in the final ones ensures that the partition is reasonably well balanced, while minimization of the vertex cut within the middle partition ensures that this cut is reasonably small.
A similar approach was taken in \cite{DBLP:conf/ipps/DellingGRW11}.

% \begin{figure}[t]
% \begin{tikzpicture}
% % vertices
% \foreach \pos/\name/\tag in {%
% {(0.4,2)/C/~}, {(2,1.6)/D/~}, {(3.6,2)/E/~},
% {(0,1)/A}, {(1.2,1)/F/~}, {(2.8,1)/G/~}, {(4,1)/B},
% {(0.4,0)/H/~}, {(2,0.4)/I/~}, {(3.6,0)/J/~}}
%     \node[vertex] (\name) at \pos {\tag};
% % edges
% \foreach \source/\dest in {%
% A/C, A/F, A/H, B/E, B/G, B/J, C/D, D/E, D/G, F/I, G/J, H/I, I/J}
%     \path[edge] (\source) -- (\dest);
% % partitions
% \draw[dotted,thick] (-0.4,-0.4) rectangle ++(1.2,2.8) node[above left=2mm] {$P'_A$};
% \draw[dotted,thick] (0.9,-0.4) rectangle ++(2.2,2.8) node[above=5mm,left=0mm] {wide separator};
% \draw[dotted,thick] (3.2,-0.4) rectangle ++(1.2,2.8) node[above left=2mm] {$P'_B$};
% \draw[dotted,thick] (2,1) ellipse (5mm and 10mm) node[above=10mm] {vertex cut};
% \end{tikzpicture}
% \caption{Bi-Partition using Vertex Cut}\label{fig:vertex-cut}
% \end{figure}

\begin{figure}[t]
\centering
\includegraphics[scale=0.45]{img/rough_partition.pdf}
\begin{center}
$S$\hspace{3cm}$T$    
\end{center}
\caption{Bi-Partition using Vertex Cut.}
\label{fig:vertex-cut}
\end{figure}
\end{comment}

\begin{comment}
Our partitioning Algorithm consists of four steps that are described in detail in the following,

\vspace{0.1cm}
\noindent\textbf{Step 1.~}We start with two vertices A and B as far apart as possible. For this we pick an arbitrary vertex A', find B as a vertex with maximal distance from A', and finally find A as a vertex with maximal distance from B. While this approach does not ensure optimality it is fast, requiring just two BFS or Dijkstra searches.

\vspace{0.1cm}
\noindent\textbf{Step 2.~}We assign to each vertex $v$ a \emph{partition weight} of
\[
pw(v) := \dist(A,v) - \dist(B,v)
\]
Here distances to $B$ have already been computed while finding $A$, while distances to $A$ can be found with one additional search.
The initial partitions $P'_A$ and $P'_B$ are then created by picking vertices with lowest and highest partition weights, respectively, until the desired size (e.g. 30\%) is reached.
Remaining vertices make up the wide separator.

\vspace{0.1cm}
\noindent\textbf{Step 3.~}We find a minimal vertex cut within the wide separator. For this, we contract all vertices in partitions $P'_A$ and $P'_B$ into single vertices $S$ and $T$, respectively. Here $S$ is adjacent to a vertex $v$ in the wide separator iff any vertex in $P'_A$ is, and similar for $T$. This turns the problem into a minimal (S,T)-vertex-cut problem, which can be solved in polynomial time.
For this we first reduce the problem to a maximum flow problem using the well-known graph transformation depicted in Figure~\ref{fig:transform}, copied from \cite[p. 205]{Bondy1976}.
We then employ Dinic's algorithm \cite{DBLP:conf/birthday/Dinitz06} to solve it.

\begin{figure}[t]
\includegraphics[width=\columnwidth]{st-vertex-cut-transform.png}
\caption{Reducing min vertex cut to max flow \cite{Bondy1976}}\label{fig:transform}
\end{figure}

\vspace{0.1cm}
\noindent\textbf{Step 4.~}Once a vertex cut has been found and removed from the graph, we assign connected components containing vertices in $P'_A$ or $P'_B$ to $P_A$ or $P_B$, respectively.
Should a connected component not contain vertices from either $P'_A$ or $P'_B$, then these are assigned to the smaller sub-partition to improve balance.

\vspace{0.1cm}


To find a minimal vertex cut within the middle partition, we contract all vertices in partitions $P'_A$ and $P'_B$ into single vertices $S$ and $T$, respectively.
Here $S$ is adjacent to a vertex $v$ in the middle partition iff any vertex in $P'_A$ is, and similar for $T$.
This turns the problem into a minimal (S,T)-vertex-cut problem, which can be solved in polynomial time.
For this we first reduce the problem to a maximum flow problem using the well-known graph transformation depicted in Figure~\ref{fig:transform}, copied from \cite[p. 205]{Bondy1976}.
We then employ a specialized version of Dinic's algorithm \cite{DBLP:conf/birthday/Dinitz06} to solve it.

\begin{figure}[t]
\includegraphics[width=\columnwidth]{st-vertex-cut-transform.png}
\caption{Reducing min vertex cut to max flow}\label{fig:transform}
\end{figure}

Once a vertex cut has been found and removed from the graph, we assign connected components to either $P'_A$ or $P'_B$ while maximizing balance.
Note that when extracting a minimal vertex cut from the maximal flow found, we have two obvious options: pick for each flow path the node closest to $S$ (amongst those that cannot be reached from $S$ in the residual graph), or the node closest to $T$ (amongst those that cannot reach $T$ in the residual graph).
We evaluate both options and pick the more balanced one.

One more issue needs to be addressed. If two vertices $a\in P'_A$ and $b\in P'_B$ are directly connected by an edge, then the middle partition does not actually contain a vertex cut set, and $S$ and $T$ end up with an edge between them.
In that case -- which occurs mostly at the lower levels of the partitioning tree -- we move both $a$ and $b$ to the middle partition, and connect them to $S$ and $T$ respectively.
This ensures that one of them will become a cut vertex, while the other will be assigned to its original partition, which is important to maintain balance guarantees.

Pseudo code for this approach is given as Algorithm~\ref{algo:partition}.

\begin{algorithm}[t]
\caption{Partition}\label{algo:partition}
\SetCommentSty{textit}
\SetKwFunction{FMain}{Partition}
\SetKwFunction{FRough}{RoughPartition}
\SetKwProg{Fn}{Function}{}{end}
\Fn{\FMain{$G$, $\beta$}}{
%    \tcp{find distant nodes using BFS}
%    $A\gets$ node furthest away from arbitrary node\\
%    $B\gets$ node furthest away from A\\
%    \tcp{find rough partitions}
%    sort nodes by $d_G(A,v) - d_G(B,v)$\\
%    $P'_A\gets$ first $\beta\cdot|V|$ nodes\\
%    $P'_B\gets$ last $\beta\cdot|V|$ nodes\\
%    $C\gets V\setminus(P'_A\cup P'_B)$\\
    $(P'_A,C,P'_B)\gets\FRough(G,\beta)$ \\
    \tcp{find vertices in cross-partition edges}
    $C_A\gets P'_A\cap N(P'_B)$\\
    $C_B\gets P'_B\cap N(P'_A)$\\
    \tcp{construct s-t flow graph}
    $G_{ST}\gets G[C\cup C_A\cup C_B]\cup \{s,t\}$\\
    $N_S\gets C_A\cup \big(C\cap N(P'_A\setminus C_A)\big)$\\
    $N_T\gets C_B\cup \big(C\cap N(P'_B\setminus C_B)\big)$\\
    \ForEach{$v\in N_S$}{
        add edge $(s,v)$ to $G_{ST}$\\
    }
    \ForEach{$v\in N_T$}{
        add edge $(t,v)$ to $G_{ST}$\\
    }
    \tcp{find minimum cut (Dinic's algorithm)}
    $\vcut\gets$ minimum s-t vertex cut on $G_{ST}$\\
    \tcp{construct final partitions}
    $CC\gets$ connected components of $G\setminus\vcut$\\
    \ForEach{$cc\in CC$ in order of decreasing size}{
        add $cc$ to smaller of $P_A$, $P_B$\\
    }
    \Return $(P_A,\vcut,P_B)$
}
\end{algorithm}

\subsection{Rough Partitioning}

To find the initial rough partition, we start with two vertices A and B as far apart as possible.
For this we pick an arbitrary vertex, find A as a vertex with maximal distance from it, and finally find B as a vertex with maximal distance from A.
While this approach does not ensure optimality it is fast, requiring just two BFS or Dijkstra searches (both work equally well).

Next, we assign to each vertex $v$ a \emph{partition weight} of
\[
pw(v) := \dist(A,v) - \dist(B,v)
\]
%Here distances to $B$ have already been computed while finding $A$, while distances to $A$ can be found with one additional search.
The initial partitions $P'_A$ and $P'_B$ are then created by picking vertices with lowest and highest partition weights, respectively, until the desired size (e.g. 30\%) is reached.
Remaining vertices make up the middle partition.

However, there is again a complication that needs to be addressed.
Partition weights partition the vertex set into equivalence classes, and it can happen that an equivalence classe becomes so big that it intersects with both $P'_A$ and $P'_B$ (and contains the middle partition entirely).
Such a case is depicted in Figure~\ref{fig:bottleneck}, where $v$ constitutes a bottleneck that causes all vertices past it to have the same partition weight as $v$.
As a result, nodes from this equivalence class are added to $P'_A$ and $P'_B$ arbitrarily, leading to huge cuts.

\begin{figure}[t]
\begin{tikzpicture}
% vertices
\foreach \pos/\name/\tag in {%
{(0,2)/A}, {(1,2)/C/~}, {(2,2)/V/v}, {(3,2)/D/~}, {(4,2)/B},
{(1,1)/E/~}, {(2,1)/F/~}, {(3,1)/G/~},
{(1,0)/H/~}, {(2,0)/I/~}, {(3,0)/J/~}}
    \node[vertex] (\name) at \pos {\tag};
% edges
\foreach \source/\dest in {%
A/C, C/V, V/D, D/B, V/E, V/G, E/F, E/H, F/G, F/I, G/J, H/I, I/J}
    \path[edge] (\source) -- (\dest);
\end{tikzpicture}
\caption{Bottleneck ``breaking'' partition weights}\label{fig:bottleneck}
\end{figure}

To address this issue, we first identify the bottleneck as the vertex (or vertices) within the equivalence class closest to $A$ and $B$.
Figure~\ref{fig:bottleneck} suggest using this bottleneck as a cut.
However, in general it may not disconnect the graph, and even if it does, the resulting partition may not be balanced.
Instead we remove the bottleneck from the graph temporarily and repeat the process for finding a rough partition on the remaining graph.
The bottleneck itself it then added to the wide cut.

As this bottleneck removal can lead to the graph being disconnected, we need to ensure that disconnected graphs are handled properly.
For this, we first compute the connected components of $G$.
If the largest component $C_{\max}$ contains no more than $(1-\beta)\cdot|V|$ nodes, the empty cut is already balanced.
Otherwise we find our rough partition within $C_{\max}$.

Pseudo code for this approach is given as Algorithm~\ref{algo:rough-partition}.

\begin{algorithm}[t]
\caption{Rough Partition}\label{algo:rough-partition}
\SetCommentSty{textit}
\SetKwFunction{FMain}{RoughPartition}
\SetKwProg{Fn}{Function}{}{end}
\Fn{\FMain{$G$, $\beta$}}{
	\If{$G$ is disconnected} {
	    $CC\gets$ connected components of $G$\\
		$C_{\max}\gets$ largest connected component\\
		\If{$|C_{\max}| > (1-\beta)\cdot |V|$}{
			$(P'_A,C,P'_B)\gets\FMain(C_{\max},\beta)$ \\
			\Return $(P'_A,\; C\cup(V\setminus C_{\max}),\; P'_B)$
		}
		\Else {
		    \ForEach{$cc\in CC$ in order of decreasing size}{
                add $cc$ to smaller of $P_A$, $P_B$\\
		    }
		    \Return $(P_A,\emptyset,P_B)$
		}
	}
    \tcp{find distant nodes using BFS}
    $A\gets$ node furthest away from arbitrary node\\
    $B\gets$ node furthest away from A\\
    \tcp{find rough partitions}
    sort nodes by $pw(v)=d_G(A,v) - d_G(B,v)$\\
    $P'_A\gets$ first $\beta\cdot|V|$ nodes\\
    $P'_B\gets$ last $\beta\cdot|V|$ nodes\\
	\tcp{handle bottlenecks}
	$w_A\gets\max\{pw(v) \mid v\in P'_A\}$\\
	$w_B\gets\min\{pw(v) \mid v\in P'_B\}$\\
	\If{$w_A = w_B$}{
		$EQ\gets \{ v\in V \mid pw(v) = w_A\}$
		$\mathcal{B}\gets \arg\min_{v\in EQ} d_G(A,v)$\\
		$(P'_A,C,P'_B)\gets\FMain(G\setminus\mathcal{B},\beta)$\\
		\Return $(P'_A,C\cup\mathcal{B},P'_B)$
	}
    $C\gets V\setminus(P'_A\cup P'_B)$\\
    \Return $(P'_A,C,P'_B)$
}
\end{algorithm}

\subsection{Distance Preservation}
%\q{(we need to formalise several observations here more formally and then illustrate them via examples.)}
After partitioning a graph $G$ into $P_A, P_B$ and cut set $\vcut$, we need to ensure that distances within $P_A$ and $P_B$ remain the same as distances within $G$.

\begin{definition}
A partition $P \in \{ P_{A}, P_{B} \}$ is distance preserving with respect to $G$ if for all $u, v \in V(P)$, $d_{P}(u,v) = d_{G}(u,v)$. A NB tree decomposition is distance preserving if every partition is distance preserving with respect to its parent graph.
\end{definition}

This definition gives us an important result in Lemma \ref{lem:distance_preservation}, which can be proved trivially.

\begin{lemma}
Given a distance preserving NB tree decomposition, every partition $P_{i}$ is distance preserving with respect to the input graph $G$.
\label{lem:distance_preservation}
\end{lemma}

We motivate how distance preservation is achieved using Lemma \ref{lem:shortcut}.


\begin{lemma}
For any two vertices $x,y$ within the same partition $P \in \{ P_A, P_B \}$ and $\dist_P(x,y)\neq\dist_G(x,y)$, all shortest paths between $x$ and $y$ must pass through vertices outside of $P$. In particular, this means that all shortest paths must pass through two or more distinct vertices in $P$ incident to $\vcut$.
\label{lem:shortcut}
\end{lemma}

\begin{example} An example illustrates the above case...
\end{example}

We shall refer to vertices in $P$ incident to $\vcut$ as \emph{border} vertices.

\begin{definition}[Border Vertex]
A vertex $v \in P$ is a border vertex if for any $w \in \vcut$, $v \in N_{G}(w)$. 
\end{definition}

It would thus suffice to insert a \emph{shortcut} edge between each pair of border vertices, with edge weight equal to their distance in $G$.
Then for each shortest path between $x$ and $y$ in $G$ there exists a path of equal length that lies entirely in $P$, so distances are preserved. \textcolor{red}{(Already have $B$ for maximum distance vertices, so either change, or need different letter for border vertices)}.

\begin{lemma}
Given a partition $P$ with parent $G$ and border vertices $Border(P)$, we can create a distance preserving partition $P'$ as:
\begin{itemize}
    \item $V(P') = V(P)$
    \item $E(P') = E(P) \cup \{ (b_{i}, b_{j}) \ | \ b_{i} \ne b_{j}, b_{i}, b_{j} \in Border(P) \}$ where $w(b_{i},b_{j}) = d_{G}(b_{i},b_{j})$
\end{itemize}
\end{lemma}

\begin{example} An example illustrates the above case...
\end{example}

However, not all of these shortcuts are actually needed. The following Lemma characterise redundant shortcuts:

\begin{lemma}
A shortcut between $b_1,b_2$ is redundant iff
\begin{enumerate}
\item $\dist_G(b_1, b_2) = \dist_P(b_1, b_2)$, or
\item $\dist_G(b_1, b_2) = \dist_G(b_1, b_3) + \dist_G(b_3, b_2)$ for some border vertex $b_3\notin\{b_1, b_2\}$.
\end{enumerate}
\end{lemma}

We compute distances between pairs of border vertices in $P_A$ or $P_B$ by performing one Dijkstra search for each border vertex (one border vertex per partition can be skipped). To obtain distances in $G$, we apply formula (\ref{eq:dist}) to get the length of shortest paths passing through one or more cut vertices.
The distance in $G$ is then the minimum of that and their distance in $P_A$ or $P_B$. Once distances between all pairs of border vertices in $G$ and $P_A/P_B$ have been computed, checking conditions (i) and (ii) becomes trivial.
Pseudo code for this approach is given as Algorithm~\ref{algo:shortcuts}.

\begin{algorithm}[t]
\caption{Add Shortcuts}\label{algo:shortcuts}
\SetCommentSty{textit}
\SetKwFunction{FMain}{AddShortcuts}
\SetKwProg{Fn}{Function}{}{end}
\Fn{\FMain{$G$, $\vcut$, $P$}}{
    $B\gets N_G(\vcut)\cap P$ \\
    \ForEach{$b\in B$}{
        run Dijkstra in $P$ starting from $b$ \\
        \ForEach{$b'\in B\setminus\{b\}$}{
            store $d_P(b,b')$ \\
            \tcp{distances to cut vertices already known}
            $d_{cut}\gets\min\{ d_G(v,c) + d_G(c,w) \mid c\in\vcut \}$ \\
            $d_G(b,b')\gets min(d_P(b,b'),\; d_{cut})$ \\
        }
    }
    \ForEach{$b_1,b_2\in B$}{
        \If{$d_G(b_1,b_2) < d_P(b_1,b_2)$}{
            redundant $\gets\false$ \\
            \ForEach{$b_3\in B\setminus\{b_1,b_2\}$}{
                \If{$d_G(b_1,b_3) + d_G(b_3,b_2) = d_G(b_1,b_2)$}{
                    redundant $\gets\true$
                }
            }
            \If{not redundant}{
                add shortcut $(b_1,b_2,d_G(b_1,b_2))$
            }
        }
    }
}
\end{algorithm}

\begin{example} An example illustrates the above case...
\end{example}
\end{comment}

\begin{comment}
\section{Hierarchical Cut Labelling}

\begin{definition}[Partial Vertex Order]
Let $T_G=(\mathcal{N}, \mathcal{E}, \ell)$ be a balanced tree hierarchy over $G=(V,E)$. Then $T_G$ defines a \emph{partial vertex order} $\preceq$ on $V$ such that, for any two vertices $v_i,v_j\in V$, $v_i\preceq v_j$ iff $\ell(v_i)$ is an ancestor of $\ell(v_j)$ in $T_G$. 
\end{definition}


\begin{definition}[Hierarchical Cut Labelling] A \q{2-hop labelling or distance labelling?} $L$ over $G=(V,E)$ is a \emph{hierarchical cut labelling} with respect to $T_G=(\mathcal{N}, \mathcal{E}, \ell)$ if, 
\begin{itemize}
\item[(1)] for any vertex $v\in V$ and any vertex $u$ in $L(v)$, $v\preceq u$ holds;
\item[(2)] for any two vertices $\{s,t\}\subseteq V$, the following holds: 
\begin{displaymath}
\begin{split}
{\{r|(r,\delta_{sr})\in L(s),(r,\delta_{tr})\in L(t)\}\supseteq}& LCA(\ell(s),\ell(t)).
\end{split}
\end{displaymath}
\end{itemize}
\end{definition}

The first condition states that $L$ is \emph{hierarchical} in terms of the partial vertex order $\preceq$ defined by $T_G$. The second condition requires that the set of hub vertices occurring in the labels of any two vertices must contain vertices in their lowest common ancestor in $T_G$. By the property of a balanced tree hierarchy, this also implies that the set of hub vertices between any two vertices corresponds to \q{a hierarchical cut on $G$.} 
%Conceptually, the labelling is represented by a binary tree where each non-leaf node $n$ is associated with

%\begin{itemize}
%\item a partition $P_n$ as tree nodes
%\item a set of cut vertices $C_n\subset P_n$
%\item distances $\dist(v, c)$, $\forall (v,c)\in P_n\times C_n$
%\end{itemize}

%The implementation of the labelling is as follows.

%When implementing this, we organize all data by vertex, as is standard for 2-hop based approaches. For each vertex $v$ and node $n$ with $v\in P_n$ we store $\dist(v,c)$ for all $c\in C_n$. We shall refer to these as the \emph{distance labels} associated with $v$ at level $k$, where $k$ is the level of node $n$ in the partition tree. Note that $v\in P_n$ holds precisely for the ancestors of the node $n_v$ associated with $v$ (including $n_v$), and thus for at most one node per level of the partition tree.

\subsection{Label Construction}
Assume that we are given a balanced tree hierarchy $T_G=(\mathcal{N}, \mathcal{E}, \ell)$.

\subsubsection{Naive Labelling} We start with a naive labelling algorithm to construct labels. Let $L(v)=\emptyset$ for each vertex $v\in V$ and $O$ be a \emph{partial vertex order} on $V$. Then. for each vertex $v \in V$, we conduct Dijkstra's search and add distances from $v$ to labels of all vertices $u \in V$ such that $\ell(v)$ is an ancestor of $\ell(u)$, i.e., $L(v) = L(v) \cup \{(u, d_G(u, v))\}$. \q{(Farhan, the connection between this construction and a given tree hierarchy $T_G$ is unclear)}

% Suppose we conduct Dijkstra searches from the vertices in the order of $v_1 \preceq v_2 \preceq \dots \preceq v_n$. For each vertex $v_i$


\q{Then we 
add new distance entries ... iteratively.}

\subsubsection{Canonical Labelling}
%Since vertices in $P_n$ all store distances to the same set $C_n$ of cut vertices, storing these distance in a fixed order enables correct matching of distance pairs in formula (\ref{eq:dist}).
Unlike many other 2-hop approaches -- we do not store vertex identifiers in distance labels, which reduces storage requirements by half (for node identifiers and distance values of equal size). Thus, the set of all distance labels associated with $v$ can be stored as a list of lists of distance values, with one list per node level, up to the level of the node that $v$ is associated with. Additionally we store for each vertex the node in the partition tree it is associated with. Here we encode nodes as bitstrings of varying length, with each bit describing a left/right choice on the path from the root to the node.

One may observe that distances between cut vertices of the same level are stored twice with this approach.
While the impact of this inefficiency is minor, we can avoid it entirely by truncating the list of distance values associated with a vertex after the point where it would store the distance to itself.
As a result, each cut vertex only stores distances to other cut vertices appearing earlier (for an arbitrary ordering) and itself.
While storing the distance of a cut vertex to itself is obviously redundant as well, we don't eliminate it as this would complicate querying by introducing a special case.

\subsection{Tail Pruning}

As many other labeling approaches, ours bears similarities to pruned landmark labeling \cite{akiba2013fast}, where nodes are assigned a ranking, and a label is pruned if a shortest path to its associated node passes through a node of higher rank.
In our approach pruning is implicit: after a graph as been partitioned, subsequent labeling occurs only within each partition, so paths passing through the cut are effectively pruned.
This is equivalent to assigning nodes with lower cut level a higher ranking.

There are some clear advantages to using cuts: only a fraction of the labels need to be examined when answering distance queries, and the nodes associated with distance labels need not be stored explicitly.
However, nodes within a cut effectively have equal rank, which limits pruning.
That is, if a shortest path from node $v$ to cut node $c'$ passes through another cut node $c$, storing the distance between $v$ and $c$ may not be necessary.

There are two classical approaches to address this, which we shall refer to as 2-hop and 3-hop pruning.
The former is exactly how PLL operates -- nodes are ranked and $d_G(v,c')$ is pruned if $c$ has higher rank than $c$.
As a result, formula~(\ref{eq:dist}) still holds.
However, distance labels can no longer be matched via their position in the list of labels alone, thus requiring additional information to be stored and complicating querying.

For 3-hop pruning no ranking is employed, and $(v,c')$ is always pruned.
While more effective than 2-hop pruning, formula~(\ref{eq:dist}) no longer holds.
E.g. if a shortest path from $v$ to $w$ passes through $c$ and $c'$, then $d_G(v,c')$ and $d_G(w,c)$ are both pruned, and $d_G(v,w)$ must be computed as
\begin{equation}\label{eq:dist-3hop}
\dist(v,w) = \hspace{-6mm}\min_{
\begin{array}{c}
c\in L(v)\cap\vcut \\
c'\in L(w)\cap\vcut
\end{array}
} \hspace{-6mm}
\dist(v,c) + \dist(c,c') + \dist(c',w)
\end{equation}
However, evaluating (\ref{eq:dist-3hop}) naively is expensive.
\cite{akiba2014fast} utilizes node sets that lie on a shortest path to avoid pairwise comparisons, but our cuts need not form shortest paths.
The drawbacks mentioned for 2-hop pruning obviously apply as well.

In principle, all these drawbacks could be justified if pruning is sufficiently effective.
However, as our cut sets are constructed to be fairly small, this is not the case.
We evaluated this experimentally, and found that 3-hop pruning can eliminate around 30\% of all labels, while 2-hop pruning can eliminate around 25\%.
As effectiveness of 2-hop pruning heavily depends on the ranking chosen, we record 3-hop pruning effectiveness w.r.t. each cut node, and rank nodes accordingly for 2-hop pruning.

Instead of either 2-hop or 3-hop pruning, we employ a different strategy, \emph{tail pruning}, which is even less effective than 2-hop pruning, but does not share its drawbacks.

\begin{definition}[Tail Pruning]
Given an ordering of nodes in a cut $C = \{c_1, c_2, \dots, c_k\}$, a label $L(v)$ is tail pruned by a cut node $c_i$ iff it is pruned by $\{c_j \in C \mid 0 \leq j < i\}$.
\end{definition}

First, we rank each cut node based on its 3-hop pruning effectiveness and order them by decreasing rank.
We then check for each label whether 2-hop pruning could eliminate it (this can be combined with label computation).
However, we only prune a 2-hop-pruneable label if all labels to lower-ranked cut nodes can also be pruned.
As a result, only the maximal pruneable tail of the label list is pruned for each cut, and labels can still be matched by their position in the label list.

While tail-pruning requires no changes to our index structure and query approach, it does increase index construction time, due to the need to compute distances to cut vertices twice (for 3-hop and 2-hop pruneability testing).
Our experimental results include tail-pruning -- without it, index sizes increase by $\sim$10\%, while construction times decrease by $\sim$20\%.

\subsection{Parallelization}

To speed up index construction, we can use multi-threading to parallelize certain tasks.
As indexing of different partitions can be performed independently, this offers an obvious approach - whenever we partition a (sufficiently large) subgraph, we create a new thread to index the subgraphs on the two partitions in parallel.

Unfortunately, the speedup provided by this approach is limited -- around factor 1.5 on a CPU supporting 12 physical threads.
The problem here is that most of the work is still being performed in a sequential fashion, which happens for two reasons.
First, much of the work is performed early on during the first few cuts, before parallelization kicks in.
Second, even though we are looking for balanced cuts, the size of partitions can still differ significantly.
As a result, the most expensive branch (from top to bottom) of the partition tree alone accounts for almost a third of index construction costs, none of which is reduced by partition-based parallelization.

To address the latter issue, and to some degree the former as well, we apply a second form of parallelization.
When computing distances for labels, shortcuts or pruning, we perform a Dijkstra search from each cut (or border) node.
These searches can easily be carried out in parallel, with workloads being practically identical.
Together these tasks account for the majority of index construction work.
While this does not reduce the cost for partition-tree construction, partition-based parallelization does, so the two approaches complement each other.
We must note however that effective parallelization is still limited to a handful of physical threads, as a significant part of the work (>10\%) is not or not fully parallelized -- mainly early cut computations.

\end{comment}


%\begin{proof}
%Given a distance preserving decomposition, the distance between any vertices $u,v \in P_{i}$ for any partition $P_{i}$ in the decomposition has $d_{P_{i}}(u,v) = d_{G}(u,v)$, where $G$ is the input graph. Therefore, any cut which separates $u$ and $v$ at partition $P_{i}$ must satisfy formula~(\ref{eq:dist})
%\end{proof}

\begin{algorithm}[t]
\caption{Querying $s$ and $t$ \h{-- unnecessary, this is simply returning (\ref{eq:dist})}}\label{algo:query}
\SetCommentSty{textit}
\SetKwFunction{FMain}{NB-Query}
\SetKwProg{Fn}{Function}{}{end}
\Fn{\FMain{$s, t$, $H_G$, $L_G$}}{
     $N_i \gets$ LCA($s$, $t$) \\
%    \If{$N_i$ is empty}{
%        \textbf{return} direct-distance \\
%    }
    $d \gets \infty$ \\
    \ForEach{$r \in N_i$}{
        \If{$\exists\; (r,\delta_{sr})\in L(s)$ and $(r,\delta_{tr})\in L(t)$}{
            $d \gets \min(d, \delta_{sr} + \delta_{tr})$ \\
        }
    }    
    \textbf{return} $d$   
}
\end{algorithm}


% \begin{figure*}[ht]
% \centering
% \includegraphics[scale=0.5]{img/td_lca.pdf}
% \hspace*{0.3cm}
% \includegraphics[scale=0.5]{img/nb_lca.pdf}
% \caption{TBD.}
% \label{fig:lca}
% \end{figure*}

% \begin{figure*}[ht]
% \centering
% \begin{minipage}[b]{0.65\linewidth}
% \centering
% \includegraphics[width=\textwidth]{img/td_lca.pdf}
% \end{minipage}
% \hspace{0.2cm}
% \begin{minipage}[b]{0.33\linewidth}
% \centering
% \includegraphics[width=\textwidth]{img/nb_lca.pdf}
% \end{minipage}
% \caption{TBD.}
% \label{fig:lca}
% \end{figure*}




%Unfortunately, the speedup provided by this approach is limited -- around factor 1.5 on a CPU supporting 12 physical threads.
%The problem here is that most of the work is still being performed in a sequential fashion, which happens for two reasons.
%First, much of the work is performed early on during the first few cuts, before parallelization kicks in.
%Second, even though we are looking for balanced cuts, the size of partitions can still differ significantly.
%As a result, the most expensive branch (from top to bottom) of the partition tree alone accounts for almost a third of index construction costs, none of which is reduced by partition-based parallelization.

%To address the latter issue, and to some degree the former as well, 


% \subsection{Efficient Implementation}

% \subsubsection{Minimal Vertex Cut}


% \subsubsection{Shortcuts}


% \subsection{Tree Labelling Construction}
% We explain how 2-hop labelling is computed using an NB decomposition of a road network $G$. The two main steps of the query algorithm are computing the LCA of the query pair in the decomposition, and computing the minimum 2-hop distance of the labels specified by that LCA. As such, the labelling contains a mechanism to efficiently compute the LCA, and the distance labels. Conceptually, the labelling is represented by a binary tree where each non-leaf node $n$ is associated with

% \begin{itemize}
% \item a partition $P_n$ 
% \item a set of cut vertices $C_n\subset P_n$
% \item distances $\dist(v, c)$, $\forall (v,c)\in P_n\times C_n$
% \end{itemize}

% \subsubsection{Implementation} 
% The implementation of the labelling is as follows. Since we are using a binary tree, we represent partitions using a binary string. When cutting a graph whose partition string is $s$, we get two children, and assign their partition strings as $s0$ and $s1$ arbitrarily. This means that the length of the partition string depends on the level of the partition in the decomposition. As such, we also need to store the level of a partition. This is because we cannot explicitly represent different sized binary strings. For example, the graph with partition string 0 will have a child with partition string 00, which is logically distinct. However, at the implementation level, both of these will be represented by the same value, so we need an additional value to store the length of the binary string.





% %$\langle C, \{(u,d(u,v)\}_{u\in C}\rangle)\in\mathcal{L}(v)$

% %\begin{definition}[Tree Labelling] A \emph{tree labelling} $\mathcal{L}$ is the set of labels that associate with vertices in $G$, i.e., $\mathcal{L}=\{\mathcal{L}(v)\}_{v\in V(G)}$. 
% %\end{definition}

% %\q{(We need some revision and discussion on this tomorrow. Generally, my view is that formulation at the conceptual level and data structure used in implementation should be separated, and we need both. After the formulation is settled, the related notation needs to be added as well.)}




% % We store the following information in our tree labelling,

% % \begin{itemize}
% %     \item Partition: it assigns bitstrings of varying length to the nodes in the NB tree. 
% %     \item Cut Level: this stores the level of a vertex at which it becomes a cut vertex. Level of any vertex can be in the range between 0 to 63.
% %     \item Distance Index Array: 
% %     \item Distance Array: For each vertex $v$ and node $n$ with $v\in P_n$ we store $\dist(v,c)$ for all $c\in C_n$.
% % \end{itemize}

% When implementing this, we organize all data by vertex, as is standard for 2-hop based approaches. For each vertex $v$ and node $n$ with $v\in P_n$ we store $\dist(v,c)$ for all $c\in C_n$. We shall refer to these as the \emph{distance labels} associated with $v$ at level $k$, where $k$ is the level of node $n$ in the partition tree. Note that $v\in P_n$ holds precisely for the ancestors of the node $n_v$ associated with $v$ (including $n_v$), and thus for at most one node per level of the partition tree.

% Since vertices in $P_n$ all store distances to the same set $C_n$ of cut vertices, storing these distance in a fixed order enables correct matching of distance pairs in formula (\ref{eq:dist}).
% Hence -- unlike many other 2-hop approaches -- we do not store vertex identifiers in distance labels, which reduces storage requirements by half (for node identifiers and distance values of equal size). Thus, the set of all distance labels associated with $v$ can be stored as a list of lists of distance values, with one list per node level, up to the level of the node that $v$ is associated with. Additionally we store for each vertex the node in the partition tree it is associated with. Here we encode nodes as bitstrings of varying length, with each bit describing a left/right choice on the path from the root to the node.

% One may observe that distances between cut vertices of the same level are stored twice with this approach.
% While the impact of this inefficiency is minor, we can avoid it entirely by truncating the list of distance values associated with a vertex after the point where it would store the distance to itself.
% As a result, each cut vertex only stores distances to other cut vertices appearing earlier (for an arbitrary ordering) and itself.
% While storing the distance of a cut vertex to itself is obviously redundant as well, we don't eliminate it as this would complicate querying by introducing a special case.

\begin{comment}
    

\section{Theoretical Analysis}
In the following we establish some simple bounds on the time and space requirements of our approach.
For this we won't distinguish between sets and their sizes, provided the intended meaning is clear from the context.
In particular, we denote the number of vertices and edges in $G=(V,E)$ by $V$ and $E$ as well.
Additionally, given a partition tree, we define its \emph{average weighted cut size} as
\[
\vcutavg := \frac{\sum P_n \cdot C_n}{\sum P_n}
\]
Crucially, vertex cuts tend to be fairly small for road networks.
E.g. for the New York dataset with 264k vertices, the average weighted cut size was just 11.

%\subsection{Partition Tree Height}

%When computing a vertex cut, the initial partitions $P'_A,P'_B$ contain $\omega\cdot P_n$ vertices each (rounded up), where $P_n$ is the (size of the) subgraph to be partitions and $0<\omega\leq\nicefrac{1}{3}$ is a configuration parameter. Since vertices in $P'_A$ end up in either $P_A$ or the vertex cut set, $P_B$ will contain at most $(1-\omega)\cdot P_n$ vertices (dito for $P_A$). Thus the size of partitions at level $k$ is at most $V\cdot(1-\omega)^k$, and the height of the partition tree is limited by $\log_\beta(V)$ with $\beta=1/(1-\omega)$.

%\q{(this paragraph needs to be removed to somewhere else - maybe Section 8)} In particular this means that for $\omega=\nicefrac{1}{3}$ and graphs containing no more than $\nicefrac{2}{3}^{-64}\approx 186$ billion vertices, the partition tree height is limited to 64, allowing us to implement bitstrings as 64-bit integers.
%Values of $\omega>\nicefrac{1}{3}$ are possible, but an exception will need to be made for very small subgraphs (e.g. $P_n=3$) to ensure disjoint $P'_A,P'_B$ can be constructed.
%The impact of this exception on partition tree height is marginal, though it complicates the analysis.

\subsection{Vertex Cuts}

When computing a vertex cut $C_n$ for $P_n=(V_n,E_n)$, initial partitioning requires a few searches and one sort, all of which can be performed in $O(E_n\cdot\log V_n)$.
For finding a minimal (S,T)-vertex cut we employ Dinitz' algorithm \cite{DBLP:conf/birthday/Dinitz06}.
This requires at most $O(E_n\cdot C_n)$ time, since each iteration can be performed in $O(E_n)$ and increases the total flow by at least one.
Thus the total cost of computing $C_n$ is $O(E_n\cdot(\log V_n + C_n))$.

Consider now the costs for all vertex cuts at one level $k$ of the partition tree.
Since no edge of the initial graph appears in more than one partition at level $k$, the total cost for computing vertex cuts at level $k$ is bounded by $O(E\cdot(\log V + \vcutavg'))$.
Here $\vcutavg'$ denotes the average weighted cut size\footnote{
Strictly speaking, $\vcutavg'$ is weighted by number of edges, while $\vcutavg$ is weighted by number of vertices.
In practice this difference is negligible though, and we will ignore it for the sake of simplicity.
} at level $k$.
The total number of levels is bounded by $\log_\beta(V)$, as established earlier.
Thus all vertex cut computations can be performed in
\[
O(E\cdot\log V\cdot(\log V + \vcutavg))
\]

One issue we have neglected so far is that of shortcuts, as these can increase the number of edges present in lower-level partitions.
The proper complexity for computing all vertex cuts is thus
\[
O((E+S)\cdot\log V\cdot(\log V + \vcutavg))
\]
where $S$ is the total number of shortcut edges inserted.
We note however that $S<\!<E$ in practice.

\subsection{Shortcuts \& Labels}

\newcommand{\borderavg}{\widetilde{B}}

Finding shortcuts between border vertices within $P_n$ requires one search per border vertex, and thus can be performed in
\[
O(E_n\cdot\log V_n\cdot B_n)
\]
where $B_n$ is the total number of border vertices in $P_A,P_B$.
Using again that edge sets within each level of the partition tree are disjoint, this leads to an overall complexity of
\[
O(E\cdot\log^2 V\cdot\borderavg)
\]
where $\borderavg$ is a weighted average of border sizes.

Observe though that road networks contain no high-degree vertices -- experimentally, we found that most cut vertices have only degree 2 or 3, including previously added shortcuts.
Thus it makes sense to assume that the (weighted average of the) degree of cut vertices is bounded by some constant $d_{\max}$.
Then $\borderavg$ is bounded by $d_{\max}\cdot\vcutavg$, and the overall complexity bound becomes
\begin{equation}\label{eq:construction-complexity}
O(E\cdot\log^2 V\cdot\vcutavg)
\end{equation}

Computing distances in $G$ and identifying redundant shortcuts adds another term of $O(\borderavg^2\cdot(\vcutavg+\borderavg)\cdot\log V)$.
It could be avoided by searching over all of $G$ for each border vertex and tracking whether paths leave the partition or pass through other border vertices, but in practice such an approach takes longer as cuts are small.

Computation of distance labels requires one search per cut vertex, and thus leads to the same complexity bound.
We note that (\ref{eq:construction-complexity}) also dominates the time required for vertex cut construction, and thus provides a bound for total index construction time.

\subsection{Labelling Size}

The number of distance labels constructed for partition $P_n$ is precisely $P_n\cdot C_n$.
Applying the same per-level analysis as for vertex cuts, we find that the total number of labels is bounded by
\[
V\cdot\log_{\beta}(V)\cdot\vcutavg
\]
Additional storage costs include bitstrings identifying the associated partition, as well as overheads for storing the lengths of lists.
These are bounded by $O(V)$ and $O(V\cdot\log V)$ though, so
\begin{equation}\label{eq:index-size}
O(V\cdot\log V\cdot\vcutavg)
\end{equation}
bounds the total storage requirements for our index.

\end{comment}


\begin{comment}

\subsection{Proof of Correctness}

\subsubsection{Without-Shortcut Query Correctness}
\begin{proof}
Given a non-distance preserving decomposition and query vertices $u$ and $v$, let $P_{i}$ be the LCA of $u$ and $v$ in the decomposition, and let $G$ be the input graph. There are two cases:
\begin{itemize}
    \item If there is a shortest path in $G$ which is wholly contained in $P_{i}$, then querying the LCA is sufficient to compute $d(u,v)$.
    \item Otherwise, every shortest path must contain some border vertices in the border set of $P_{i}$, that is, the cut which separates $P_{i}$ from its sibling partition. Since the labels for these are stored in $L(u)$ and $L(v)$, we can reduce the correctness of the $u-v$ query from computing the 2-hop distance at $P_{i}$ to computing the 2-hop distance at the parent of $P_{i}$.
\end{itemize}
\end{proof}

\subsection{Complexity Analysis}
\end{comment}

==> section_BackgroundandRelatedWork.tex <==
%\section{Related Work}
\medskip
\noindent\textbf{Related Work.~}
In this section, we review the existing work for answering shortest-path distance queries in road networks.

%\subsection{Search-based Approaches}
\medskip
\noindent\emph{\underline{Search-based Approaches.}} A traditional approach for shortest-path distance computation in a non-negative weighted road network is Dijkstra's algorithm \cite{tarjan1983data}. This computes distance between any arbitrary pair of vertices in $O(|E| + |V|log|V|)$ time which is very slow in reality, particularly for pairs of vertices that are far apart from each other, making the search space extremely large. To improve search efficiency, a bidirectional scheme can be used to run two Dijkstra's searches: one from the source vertex and the other from the destination vertex \cite{Pohl1969BidirectionalAH}. However, these traditional approaches fail to achieve desired response time performance required by many real-world applications that operate on large road networks. 

% Many approaches \cite{geisberger2008contraction, goldberg2005computing, bast2006transit} have been designed to overcome this weakness by directing the search space towards particular vertices, rather than allowing an unrestrained search. Unfortunately, these algorithms still have problems with road networks, since a pruned search for long distance queries may still need to traverse many vertices.
To improve querying, the existing solutions accelerate searching through a pre-computed index. For example, ALT \cite{goldberg2005computing} pre-computes a partial distance index to accelerate the A* search. The hierarchical techniques have also been used to make searching faster. HiTi \cite{jung2002efficient} constructs a hierarchical structure  through graph decomposition techniques to accelerate query performance. Highway Hierarchies \cite{10.1007/11561071_51} and Contraction Hierarchies \cite{geisberger2008contraction}  have shown to prune the search space massively for efficient querying. Moreover, algorithms such as Transit Node Routing \cite{arz2013transit}, TRANSIT \cite{bast2006transit} and Arterial Hierarchy \cite{10.1145/2463676.2465277} integrate coordinate information and divide the map into grids to accelerate searching.

%\smallskip
%\noindent\textbf{Contraction Hierarchies (CH).~}Contraction hierarchies approach proposed in \cite{geisberger2008contraction} defines a total order among vertices as a vertex hierarchy by assigning each vertex $v$ a rank $r(v)$ using some predefined criteria and then applies a shortcut operation to each vertex in this order. When preprocessing a vertex $v$, the shortcut operation temporarily removes $v$ from the graph and adds shortcut edges between its neighbors to preserve the distance information. The output of contraction hierarchy algorithm is a graph $G^+ = (V, E \cup E^+)$ (where $E^+$ is the set of shortcut edges added) and the topological order of a graph. While distance computation, their method only searches edges $(u, v)$ where $v$ is of higher-rank than $u$ in $G^+$ and thus massively prunes the search space.

% Contraction Hierarchies (CH) \cite{geisberger2008contraction} perform a directed search where edges are searched based on a hierarchical structure. At preprocessing time, the method constructs artificial edges known as shortcuts which traverse many vertices, and allow the search to jump large parts of the network quickly. These shortcut edges are arranged in a hierarchy which determines the order in which they are searched at query time. Importantly, the method only searches edges in increasing importance in the hierarchy. This massively prunes the search space, and directs the search towards shortcuts, which is important for computing long distance queries efficiently.



%\smallskip
%\noindent\textbf{Arterial Hierarchy (AH).~}Zhu et al. proposed the \emph{Arterial Hierarchy} \cite{10.1145/2463676.2465277} approach as an improvement to CH algorithm. Unlike CH, AH algorithm exploits 2-dimensional spatial properties on a network and creates shortcuts using $4\times 4$ grids. Query processing of AH is similar to that of CH, i.e., it searches from lower-ranked vertices to higher-ranked vertices. AH has shown to outperform CH when answering distance queries since it consumes both network information and spatial information.

These algorithms are limited to perform well for short-distance queries. For long-distance queries, their search space is still large, and computation is expensive even with large amounts of pruning. %As before, this is a significant problem for road networks, and motivates solutions which can answer queries efficiently even when they are very far apart.

\smallskip
\noindent\emph{\underline{Labelling-based Approaches.}}
To address the limitations of search-based approaches, labelling-based approaches for road networks have been studied with great success \cite{abraham2011hub,abraham2012hierarchical,ouyang2018hierarchy,akiba2013fast,chen2021p2h,jin2012highway}. Labelling-based methods rely on a pre-computed index that stores the distance information for all pairs of vertices in a road network. Most of the existing methods pre-compute an index that satisfies 2-hop cover property \cite{cohen2003reachability} which requires at least one common vertex in $L(s)$ and $L(t)$ to be on a shortest-path between any query pair $(s, t)$. They provide a significant advantage for long-distance queries, and allow us to compute distances with fewer operations. We will discuss main existing approaches in detail in Section~\ref{sec:existing-solutions}.

% Most practical labelling-based approaches use either 2-hop or 3-hop labelling. 2-hop labelling \cite{ouyang2018hierarchy, chen2021p2h, akiba2013fast} relies on the property that for any query pair $(s,t)$, we can compute $d(s,t) = \min_{i} (d(s,w_{i}) + d(w_{i},t))$. Specifically, every pair of vertices will have some set of matching labels, and we can compute the distance between those vertices using only those matching labels. 3-hop labelling \cite{akiba2014fast, jin2012highway} relaxes this matching, and computes query distances as $d(s,t) = \min_{i,j} (d(s,w_{i}) + d(w_{i},w_{j}) + d(w_{j},t))$. It can be seen how this will generally be slower for answering distance queries than 2-hop approaches. However, the relaxed conditions for matching mean that we can store potentially fewer labels, and therefore save on the memory size of the labelling.


%\smallskip
%\noindent\textbf{Hub Labelling (HL).~}In \cite{abraham2011hub,abraham2012hierarchical}, Abraham et al. proposed a hub-based labelling algorithm which aims to use distances to hub vertices as the label of a vertex. During a label generation process, for a given vertex $v$, their algorithm runs a forward CH search and a backward CH search \q{on $G^+$} from $v$ and adds \q{visited vertices and their distances to $v$} into $L_f(v)$ and $L_b(v)$, respectively. Then, given any two vertices $s$ and $t$, the intersection of $L_f(s)$ and $L_b(t)$ contains \q{the maximum-rank vertex $u$} on a shortest-path between $s$ and $t$, and $\delta(s, u) + \delta(u, t)$ is the shortest-path distance from $s$ to $t$. Further, it reduces the size of labels by removing vertices $w$ from $L_f(v)$ and $L_b(v)$ if $\delta(v, w) > d_G(v, w)$. More precisely, if a vertex $u \in L_f(s) \cap L_b(t)$ with $\delta(s, u) = d_G(s, u)$ and $\delta(u, t) = d_G(u, t)$, $u$ is not removed. The quality of the labelling depends on the vertex order for contraction hierarchy. 

%\smallskip
%\noindent\textbf{Pruned Highway Labelling (PHL).~}Akiba et al. \cite{akiba2014fast} proposed \emph{pruned highway labelling} method which aims to store distances to paths instead of hubs in the labels for each vertex. Their algorithm first decomposes a road network into disjoint shortest paths and then computes a label for each vertex $v$, which contains the distance from $v$ to vertices in a small subset of the computed paths. Using these labels, a distance query $d_G(s, t)$ can be answered by hopping from $s$ to a path starting from a vertex $u \in L(s) \cap L(t)$ and then hopping from the path to $t$. They use pruned landmark labelling technique \cite{akiba2013fast} in indexing to reduce the label size.

%These methods may not perform well for short-distance queries due to their large label sizes and thus result in performing unnecessary computations. Dian et al. \cite{ouyang2018hierarchy} addresses the limitations of search-based and labelling-based methods using tree decomposition based approach to compute vertex hierarchies and 2-hop labelling.

%\smallskip
%\noindent\textbf{Hierarchical 2-Hop Labelling (H2H).~}Dian et al. \cite{ouyang2018hierarchy} proposed \emph{Hierarchical 2-Hop Index} (H2H-Index) which has shown to outperform previous state-of-the-art methods, including hub labelling method and pruned highway labelling method. The general idea of this method is to design a label for each vertex as well as a hierarchy among all vertices in a road network. Then, it answers a shortest distance query $d_G(s, t)$ without exploiting all vertices in the labels of $s$ and $t$, and only visit a subset of vertices in the labels of $s$ and $t$ attentively with the help of the vertex hierarchy. Intuitively, when the distance between $s$ and $t$ is small which can be achieved with the assistance of a vertex hierarchy, only a small subset of vertices in the labels of $s$ and $t$ need to be visited and thus resulting in faster query processing time.

% There are a number of challenges with labelling-based approaches. The first is ensuring that the labels can correctly construct the true query distance. One way to do this is to use vertex cuts as the basis for labels \cite{ouyang2018hierarchy, chen2021p2h}. A vertex cut is a set of vertices which disconnects a graph when removed. This gives them an important property which is useful for labelling. Given a vertex cut $C$ which partitions a graph $G$ into components $G_{1}, G_{2}, \dots, G_{k}$, any path between $u \in V(G_{i})$ and $v \in V(G_{j})$ with $i \ne j$ must pass through some cut vertex $c \in C$. Therefore, given a vertex cut, we can use the vertices in that cut to give a partial 2-hop labelling which will be sufficient to answer distance queries for any pair of vertices in different components. However, it cannot answer queries for vertices in the same partition. This raises the challenge of being able to create cuts such that for any pair of vertices, there is some cut which separates then, and can be used to give a 2-hop distance between those vertices.

% Several existing solutions use a tree decomposition (TD) approach to assign a tree-structured hierarchy to all vertices in a road network~\cite{ouyang2018hierarchy,chen2021p2h}. 


% \textbf{P2H:}
% There are a number of drawbacks to H2H. Most importantly, due to the complex structure of the tree decomposition, it is difficult to minimise the sizes of cuts given by the decomposition. Since the sizes of cuts affects both the labelling size and the query performance, it is critical to ensure that cuts are as small as possible. An extension of H2H known as P2H \cite{chen2021p2h} partially addresses this by using pruning techniques to reduce the effective label size. In H2H, vertices are queried by finding their lowest common ancestor (LCA) in the decomposition, and using the vertices stored at that LCA as a vertex cut. P2H notes how the tree structure can be leveraged to reduce the number of searched labels. However, this does not reduce the number of labels which need to be stored, so the pruning only affects query times. \q{(I removed this paragraph from Section 3.1 because it seems that including it there indicates that we need to compare our method with P2P in the experiments.)}

%\smallskip
%\noindent\textbf{Our approach.}
%This leaves us with a fundamental question: how do we leverage the important properties of H2H while allowing room for optimisation of cuts. From P2H, we see that relying on the tree decomposition still has limitations to what can be optimised, and how much is impacted by reducing cut sizes. This motivates looking at the problem from a different perspective. Instead of using a tree decomposition which gives us cuts, we focus on finding cuts and building a decomposition from those cuts. 

%By moving from a tree decomposition to a cut focused decomposition, we aim to make it more effective to optimise cut sizes. Specifically, by minimising cuts explicitly, we aim to reduce the labelling size, and reduce the number of labels which need to be searched at query time. Using cuts, we can then build a decomposition of the input graph which maintains the important tree properties of H2H. Specifically, in order to query a pair of vertices, we only need to find their LCA in the decomposition, and use that to efficiently select a subset of labels needed to compute their 2-hop distance. 




% \begin{itemize}
%     \item 1st paragraphs: Dijkstra's algorithm and its limitations. What are the solution to address these limitations? e.g., improved search-based methods and labelling-based methods.

%     \item 2nd paragraph: A topic sentence about improved search-based methods, explain e.g., A* search, contraction hierarchy methods. Discuss their observations and limitations.

%     \item 3rd-4th paragraphs: A topic sentence about labelling-based methods, discuss HL, HCL, PHL, H2H and P2H, talk about the solutions they proposed to addressed the limitations of improved search-based methods. Discuss their key observations and drawbacks.

%     \item 5th paragraph: A topic sentence about the proposed methods, how is it different and better than state-of-the-art solutions. Also explain why the proposed method is for road networks and might not work well on complex networks.
% \end{itemize}



==> section_Introduction-OldVersion.tex <==
\section{Introduction}
The \emph{distance query} problem in road networks is to find the length of a shortest-path between any two given locations. This is one of the most fundamental problems with numerous applications such as GPS navigation \cite{goldberg2005computing}, route planning \cite{fan2010improvement}, traffic monitoring \cite{kriegel2007proximity}, and point of interest (POI) recommendation \q{\cite{?}}. Many of these applications have low latency requirements, requiring a distance query to be answered quickly, e.g., in microseconds. A traditional approach to answering a distance query is to use the Dijkstra's algorithm \cite{tarjan1983data} which can compute the length of a shortest-path from a source vertex $s$ to a destination vertex $t$ in polynomial time. To improve search efficiency, a bidirectional scheme can be used to run two Dijkstra's searches: one from the source vertex $s$ and the other from the destination vertex $t$ \cite{Pohl1969BidirectionalAH}. However, these traditional approaches are found to be highly inefficient on road networks that are regarded as having large diameters, failing to achieve real-time requirements of real-world applications that operate on road graphs. Thus, indexing-based approaches emerged as an attractive way of achieving desired response time \cite{geisberger2008contraction,arz2013transit,abraham2011hub,abraham2012hierarchical,10.1007/11561071_51,jung2002efficient,goldberg2005computing,10.1145/2463676.2465277,bast2006transit,akiba2014fast}. The purpose of these indexing-based approaches is to investigate structural properties of a road network such as low-degree and planarity, so as to process a distance query efficiently.

The current state-of-the-art indexing-based approaches \cite{abraham2011hub,abraham2012hierarchical,akiba2014fast,ouyang2018hierarchy,chen2021p2h} for the \emph{distance query} problem on road networks precompute and store shortest-path distances between pairs of vertices in an index, called \emph{distance labelling}, under certain properties such as 2-hop cover \cite{cohen2003reachability}. Such approaches usually exploit hierarchical structure of a road network and fall into three categories, hub-based labellings, highway-based labellings, and tree decomposition based labellings. The hub-based  labellings \cite{abraham2011hub,abraham2012hierarchical} \q{find a vertex hierarchy by preprocessing a road network} and then based on such hierarchy precompute a 2-hop label for each vertex in a road network. The label of a vertex $v$ contains the shortest-path distances from $v$ to a subset of vertices in the road network. The highway-based labellings \cite{akiba2014fast} decompose a road network into disjoint shortest-paths to find vertex hierarchy and then based on the computed hierarchy precompute a label for each vertex $v$ which contains the distances from $v$ to a subset of decomposed shortest-paths. For these approaches, the distance query $(s, t)$ answers the length of a shortest-path by joining the common hubs in the labels of $s$ and $t$.
The tree decomposition based labellings \cite{ouyang2018hierarchy,chen2021p2h} decompose a road network using tree decomposition techniques \cite{bodlaender2006treewidth} to find vertex hierarchy. In this approach, vertex hierarchy is not used to compute a distance labelling, rather it is used to reduce the labelling search for efficient distance querying. Specifically, the distance query $(s, t)$ selects a subset of hubs from the label sets of $s$ and $t$ with the help of hierarchy to compute the shortest-path distance between $s$ and $t$.

% Computing the shortest-path distance between two locations in a road network is a long standing problem and necessary building block of many road monitoring systems. Answering distance queries on road networks is critical for numerous applications such as GPS systems \cite{goldberg2005computing}, route planning \cite{fan2010improvement}, and traffic monitoring \cite{kriegel2007proximity}. Many of these systems rely on answering queries in real time, making traditional methods such as Dijkstra's algorithm impractical. This has led to the design of multiple algorithms which can efficiently answer shortest distance queries on large road networks. 



% Structurally, road networks are characterised by high diameter and low node degree, making search-based methods such as Dijkstra's algorithm highly inefficient. One branch of research which has seen much success is labelling-based methods \cite{ouyang2018hierarchy, chen2021p2h, akiba2013fast, akiba2014fast}. Instead of performing a query time search in the network, these methods precompute distance labels which capture distance information about the graph, and then combine them at query time to compute distances. This allows these methods to answer queries significantly faster than search-based methods, at the cost of requiring large storage sizes for the precomputed labels. As such, it is still an open problem how to design algorithms which can give both fast query times with small memory costs. 

\smallskip
\noindent\textbf{Motivation.~}From the above analysis, we observe that these approaches leverage vertex hierarchy in two ways. One way is to find a good vertex ordering to reduce the labelling size. In hub-based labellings and highway-based labellings, a distance query $(s, t)$  explore the complete label sets of $s$ and $t$ in order to compute a shortest-path distance. Therefore, they aim to find a good ordering of vertices which can produce smaller labelling, hence letting a distance query to process smaller label sets. The other way is to use a hierarchical structure e.g., tree, to assign hierarchy among vertices, and then use such vertex hierarchy on any given labelling to reduce search space on the label sets for a distance query $(s, t)$. In other words, vertex hierarchy enables a distance query to pick a subset in the labels of $s$ and $t$ to answer the query efficiently.

%Instead of using a tree decomposition which gives us cuts, we focus on minimising cuts explicitly, reduce the labelling size, and reduce the number of labels which need to be searched at query time.

\smallskip
\noindent\textbf{Our Idea.~}Our idea is to design a solution that combines the benefits of vertex hierarchy from both perspectives - leveraging a hierarchy to reduce the size of a distance labelling and also further reduce the search space on such a labelling when performing distance queries in a road network. This way we can accelerate the performance of distance queries, which are of two types in general, long-range and short-range queries. Particularly, for long-range queries, the label sets are usually large, thus by processing a very small subset of labels can improve query performance significantly, similarly performance for short-range queries further improves as well. To make our idea practically applicable, the following questions need to be addressed regarding the desirable characteristics of such a hierarchy:  1) How can such a hierarchy be designed for each vertex to reduce the overall size of a distance labelling? 2) How can such a hierarchy be used to accelerate searching on the labels sets of a distance query $(s, t)$ by processing a subset of labels from the labels of $s$ and $t$?  
% One of the recent state-of-the-art labelling-based approaches is called H2H \cite{ouyang2018hierarchy}. It uses a 2-hop labelling-based on the tree decomposition of an input graph. At query time, the tree structure allows queries to select a small subset of labels which need to be processed to answer the query. Because of this, H2H can answer distance queries significantly faster than other algorithms. However, in order to guarantee query correctness, the method requires storing a large number of labels, which gives it considerably larger memory size than many search-based methods. 

% There are two important properties given by the tree decomposition in H2H. The first is the tree structure, which makes querying extremely efficient. The second is vertex cuts, which are needed to guarantee query correctness. Importantly, the sizes of vertex cuts affects both the query performance, and the labelling size. This means it is critical to compute a tree decomposition with minimal cut sizes. However, this problem is infeasible, and so H2H relies on approximate methods which create a suboptimal decomposition. 

% The necessity for minimising cuts led to a follow up algorithm called P2H \cite{chen2021p2h} which aimed to provide additional query time pruning. While this is able to reduce query times, it does not affect the overall labelling size, so this method still has the same limitations as H2H. As such, it is still an open problem how to leverage the tree structured decomposition to give a method with both fast query times, and small memory costs.

% In this paper, we propose a fundamental change to the role of cuts in a tree decomposition. Instead of creating a tree decomposition which gives vertex cuts, we compute cuts on a graph and form a tree structure using those cuts. Optimising cuts in a tree decomposition is NP-hard. However, it is a well-known result that minimal vertex cuts can be computed on graphs in polynomial time. Computing cuts directly also lends itself well to creating a tree structure. Given a graph, we compute a cut which separates it into some number of component subgraphs. We can then compute cuts on those subgraphs, and create a tree structure from the decomposition.


% \begin{itemize}
%     \item 1st paragraph: Introducing shortest distance problem on road networks and its applications.

%     \item 2nd paragraph: What are the existing solution to solve this problem and what are the challenges. e.g. search-based solutions, labelling-based solutions.

%     \item 3rd paragraph: A topic sentence about labelling-based solutions and then discuss attempts of state-of-the-art Labelling based solutions to address the problem and their drawbacks.


%     \item 4th paragraph: Motivation - A topic sentence on the goal of this paper, i.e., tree structure based labelling for efficient querying, and explain the key observations. Why the proposed methodology developed on these observations works?

    

%     \item 5th paragraph: contributions 

%     \item 6th paragraph: empirical improvements and paper structure
% \end{itemize}


\smallskip
\noindent\textbf{Contributions.~}In this paper, we propose a new hierarchy which addresses the above questions. Our contributions are summarised as follows:

\begin{itemize}

    \item Upon analysing existing approaches that exploit hierarchical structure of road networks for efficient distance querying, we introduce a new hierarchy called \emph{balanced tree hierarchy} which enables us to reduce the size of a distance labelling significantly. We call a distance labelling computed over balanced tree hierarchy, \emph{hierarchical cut labelling (HCL)}. Further, our balanced tree hierarchy enables us to answer a distance query by processing a small subset of labels that are necessary to compute the distance. Compared to the state-of-the-art algorithms, our algorithm achieves a much faster query processing time. 

    \item We develop an efficient algorithm to construct our proposed \emph{balanced tree hierarchy}. Our algorithm recursively partitions a road network. Specifically, it first finds a balanced and minimal hierarchical cut in each partition graph and then create a minimum number of shortcuts to preserve the distance between border vertices. The result is a binary tree which defines hierarchy of all vertices in a road network.

    \item We design an efficient algorithm to construct HCL over a given balanced tree hierarchy. We discuss the drawbacks of different labellings and provide upper and lower bounds on the labelling size and then devise a novel pruning strategy, called \emph{tail pruning}, that make our proposed algorithm to produce smaller labelling that does not share the drawbacks of other labellings.

    \item We conduct extensive experiments to evaluate the performance of the proposed algorithms on 10 real-world large road networks including the whole road network of the USA. The experimental results demonstrate that our algorithm is x\% as fast as the state-of-the-art algorithms in terms of query processing while consuming x\% less labelling construction time and x\% smaller labelling size.
    
\end{itemize}
